Improving Multi-View Stereo via Super-Resolution

Today, Multi-View Stereo techniques are able to reconstruct robust and detailed 3D models, especially when starting from high-resolution images. However, there are cases in which the resolution of input images is relatively low, for instance, when dealing with old photos, or when hardware constrains the amount of data that can be acquired. In this paper, we investigate if, how, and how much increasing the resolution of such input images through Super-Resolution techniques reflects in quality improvements of the reconstructed 3D models, despite the artifacts that sometimes this may generate. We show that applying a Super-Resolution step before recovering the depth maps in most cases leads to a better 3D model both in the case of PatchMatch-based and deep-learning-based algorithms. The use of Super-Resolution improves especially the completeness of reconstructed models and turns out to be particularly effective in the case of textured scenes.

==> A2R.tex <==
%\begin{document}
%\title{Improving Multi-View Stereo\\via Super-Resolution}
%\author{\IEEEauthorblockN{Eugenio Lomurno}
%\IEEEauthorblockA{Politecnico di Milano, Italy\\
%Email: eugenio.lomurno@mail.polimi.it}
%\and
%\IEEEauthorblockN{Andrea Romanoni}
%\IEEEauthorblockA{Politecnico di Milano, Italy\\
%Email: andrea.romanoni@polimi.it}
%\and
%\IEEEauthorblockN{Matteo Matteucci}
%\IEEEauthorblockA{Politecnico di Milano, Italy\\
%Email: matteo.matteucci@polimi.it}}

%\maketitle

%\begin{figure*}[!T]
%\centering
%\includegraphics[width=0.95\textwidth]{title_picture.png}
%\end{figure*}

\vspace{0.25cm}
\begin{center}
\vspace{0.25cm}
\LARGE{Improving Multi-View Stereo Completeness via Super-Resolution}
\vspace{0.25cm}
\end{center}

\begin{center}
\Large{-- Answer to Reviewers --}
\vspace{0.25cm}
\end{center}

% \begin{center}
% Eugenio Lomurno, Politecnico di Milano \\
% eugenio.lomurno@mail.polimi.it
% \vspace{0.25cm}

% Andrea Romanoni, Politecnico di Milano \\
% andrea.romanoni@polimi.it
% \vspace{0.25cm}

% Matteo Matteucci, Politecnico di Milano \\
% matteo.matteuci@polimi.it
% \vspace{0.25cm}
% \end{center}

\begin{abstract}
This is a detailed description of the changes applied to the text in the resubmission of the paper in order to improve it with respect to the weaknesses highlighted by the anonymous reviewers. We take this opportunity to thank reviewers suggestions which have helped us in reshaping significantly the contribution which now is more clear and complete.
\end{abstract}

%\IEEEpeerreviewmaketitle

\section{Reviewer 4}
\textbf{Strength:} It is well written, and well reasoned, and the authors show a comprehensive background research and domain knowledge.

\textbf{Weaknesses:} There doesn't seem to be any novel contribution in the paper. Despite offering a well rounded study on how to combine two methods,  the main accomplishment is that it can improve results on one benchmark, and perhaps
marginally.

\begin{quote}\emph{%
As implicitly suggested by the reviewer, we have extended the evaluation of the comparison to Tanks and Temples benchmark in order to provide a more complete view on the experiments and provide better hints on the effectiveness of the Super-Resolution in improving MVS reconstructions.
}\end{quote}
There is also an assumption in the hypothesis
of the paper that might not hold true: the paper assumes
that the use of SISR can add details in the higher
resolution that can be useful for MVS, this is not
necessarily true.

\begin{quote}\emph{
With the new experiments from Tanks and Temples benchmark we show how reconstructions quality is related to images resolution.
In fact, reconstructing 3D models from downsampled versions of the original dataset leads to less accurate models than using higher resolutions.
}\end{quote}
SISR networks are highly dependant on the
dataset used for training, so unless the network was
trained on images of the same type, and more importantly
with the same resolution that the paper is targeting, the
SISR network most likely will not add much, and probably
that is why the bicubic scaling had comparable results.

\begin{quote}\emph{%
The paper was updated to address an ambiguity emerged from the reviewers comments: both the model based on Deep Learning and the bicubic upsampling are considered SISR techniques, but we deepen the use of the first as it represents the state-of-the-art in the SISR field.
The new experiments suggested by reviewers show that, given two versions of the same dataset, one in low-resolution LR of size WxH and one in high-resolution HR of size 2Wx2H, HR reconstruction always achieves much better scores than the LR version.
This answers the doubt about the assumption that adding input details improves 3D models, indeed, for both types of SISR with 2x scale factor, we have obtained better results compared with LR ones and at the same time very close to HR scores.
We agree that the training of the SISR-DL model has a great impact on the quality of the result and we assume that there is a wide improvement margin by performing fine-tuning or a complete training but still our results show how it is useful also with a general purpose training.
}\end{quote}

\paragraph{Justification} The paper is well written and thought, and has the potential of helping other papers achieve better results. But the idea is not groundbreaking nor the results very interesting. It should at least include results in more than one benchmark also.

\begin{quote}\emph{%
We are aware we are not proposing a new model, but as pointed out, the goal of this work is to propose an additional step by which create new MVS pipeline or improve existing ones down.
By extending the experimental part to the Tanks and Temples benchmark, we are expanding the pool of results with remarkable performances by applying SISR to images with low resolution paving the way for further studies on ad-hoc SISR methods capable to enhance MVS.
}\end{quote}

\section{Reviewer 2}
\textbf{Strengths:} I think that it is an interesting idea to evaluate how efficient and useful it is to apply a super-resolution technique to the input images before using a MVS algorithm. The paper is in general well written and easy to follow.

\textbf{Weaknesses:} My strongest critic is that there are no novel technical contributions in the paper. The proposed methods are straightforward combinations of off-the shelf super resolution and MVS methods. The motivation to study the
impact of super-resolution applied on input images for 3D
reconstruction is good, but technical contribution is low.

\begin{quote}\emph{%
We are aware that we are not proposing a classic technical contribution and accept the reviewer's criticism from this point of view. The intent of the paper is to create a link between two areas of research so far separated. Therefore, the proposed SR-MVS models are only a first example for a new tool and a starting point for improving the state-of-the-art in the MVS field.
Our aim is to prove with our findings this is a line of research it is worth pursuing.
}\end{quote}
The conclusion from the experimental evaluation is not
clear. In the end it seems that using or not
super-resolution and which super resolution method to use
depends a lot on the dataset. Maybe designing a new
super-resolution method that automatically adapts to the
input data for better 3D reconstruction could be an
interesting research direction. Also, because the results
depend on the method for super-resolution, experiments with
using other super-resolution methods would bee better.

\begin{quote}\emph{%
We agree with the reviewer's observation; we proceeded to modify the conclusion and enrich it with new experimental proofs.
We also agree with the comments relating to the next steps, which will surely be deepened in future works but which go beyond the purpose of this paper in which we limit ourselves to showing a type of classic super-resolution (bicubic interpolation) and one based on deep learning (DBPN) and to what extent they are beneficial to MVS.
}\end{quote}
In the experiments, the authors say that many datasets
could not be used because the input images are too high
resolution. What prevents the authors to downsample the
input images and use the downsampled images to test their
proposed method? Then it would be interesting to compare
the results obtained with the super resolution images with
those obtained with the ground truth high resolution
images. The point is to see how much artifacts are created
by the super-resolution algorithms.

\begin{quote}\emph{%
Thanks to the suggestions received, we applied the SR-MVS approach also to downsampled version of Tanks and Temples, obtaining a set of LR and HR images of the benchmark. By applying bicubic-based and deep-learning-based super-resolution to the LR images, we obtained reconstructions with scores much better than the 3D LR models and very close to the original HR ones.
As for the artifacts of the SR, these are easy to find in the starting images and become less sharp continuing in the pipeline.
It is possible to identify them, for instance, as distortions or holes in the textureless regions of 3D reconstructions from MVS PatchMatch algorithms.
}\end{quote}
I guess that there is a trade-off between processing time
and using super-resolution images as input. This should be
discussed, and the improvements in accuracy when using
super-resolution images should be balanced by the increase
in computational time.

\begin{quote}\emph{%
We agree that a temporal analysis can provide very interesting information, and we confirm that there is a kind of proportionality between the size of the input and the reconstruction time. We decided to exclude this information from the paper experiments given the heterogeneity of the input which varies by starting size, number of images and channels and by the different nature of the MVS algorithms proposed.
We believe that a comparison of this type requires a very thorough work and that it would have diverted attention from the main problem that this document aims to solve.
However, on an Intel(R) Xeon(R) CPU E5-2630 v4 @ 2.20GHz with an Nvidia GTX 1080Ti, the bicubic interpolation requires a fraction of second for image while the Deep Back-Projection Network on average requires between 2 and 10 seconds; the 3D reconstruction process is heavily affected by the number of input images; from the experiments carried out over Tanks and Temples on average SR reconstructions have required 2-3 times the time required for low-resolution ones.
}\end{quote}

\paragraph{Rating}: The motivation of the paper is interesting, but the technical contribution is low and the experimental evaluation does not allow to answer the question of the paper: “is it better to use super-resolution algorithm before applying MVS method?”. Also, some additional experiments could have been done.

\begin{quote}\emph{%
We have enriched the experimental pool with Tanks and Temples benchmark evaluation to answer the reviewer doubts.
We also reformulated the explanation of the results by focusing on the technical contribution provided and on the key points of our approach in the MVS field.
}\end{quote}

\section{Reviewer 3}
\textbf{Rating:} The authors proposed a completeness of model reconstruction by using super-resolution. The evaluation results demonstrate that the proposed method works well for
textured scenes. I suggest giving more details of
explanation of the proposed method.

\begin{quote}\emph{%
We agree with the reviewer's critic and for this reason we have enriched the experimental pool with another benchmark and discussed these new results.
We would like to clarify that the methods used are aimed at studying the effectiveness of SISR in MVS pipelines and that they do not represent the core of the paper.
}\end{quote}
It is not clear how to
design the deep back projection network to generate SISR.

\begin{quote}\emph{%
We did not elaborate on the explanation about the deep back-projection network (DBPN) design since this model has not been realized by us.
It is the SISR model built and provided by Haris \etal which is publicly available on GitHub (https://github.com/alterzero/DBPN-Pytorch).
}\end{quote}
In the evaluation results, why some low-resolution images
provide better performance? The outdoor environment
situations are different, for example, city road, highway,
urban. It is an insufficient evaluation result to apply the
proposed method to the outdoor scene applications.

\begin{quote}\emph{%
According with reviewer suggestions, we extended the proposed approach to other indoor and outdoor sequences demonstrating the connection between input images and 3D model qualities. The reason why textureless low-resolution sequences lead to better 3D models is related with the nature of both the SISR and the MVS algorithms used: PatchMatch algorithms suffer for the presence areas poor in details, SISR may produce artifacts. We shown also how CasMVSNet, the DL-MVS algorithm used in our experiments, is instead able to exploit SISR in both indoor/outdoor and textured/textureless scenarios.
}\end{quote}


% \bibliographystyle{IEEEtranS}
% \bibliography{biblio.bib}

%\end{document}

==> Improving Multi-View Stereo via Super-Resolution/A2R.tex <==
%\begin{document}
%\title{Improving Multi-View Stereo\\via Super-Resolution}
%\author{\IEEEauthorblockN{Eugenio Lomurno}
%\IEEEauthorblockA{Politecnico di Milano, Italy\\
%Email: eugenio.lomurno@mail.polimi.it}
%\and
%\IEEEauthorblockN{Andrea Romanoni}
%\IEEEauthorblockA{Politecnico di Milano, Italy\\
%Email: andrea.romanoni@polimi.it}
%\and
%\IEEEauthorblockN{Matteo Matteucci}
%\IEEEauthorblockA{Politecnico di Milano, Italy\\
%Email: matteo.matteucci@polimi.it}}

%\maketitle

%\begin{figure*}[!T]
%\centering
%\includegraphics[width=0.95\textwidth]{title_picture.png}
%\end{figure*}

\vspace{0.25cm}
\begin{center}
\vspace{0.25cm}
\LARGE{Improving Multi-View Stereo Completeness via Super-Resolution}
\vspace{0.25cm}
\end{center}

\begin{center}
\Large{-- Answer to Reviewers --}
\vspace{0.25cm}
\end{center}

% \begin{center}
% Eugenio Lomurno, Politecnico di Milano \\
% eugenio.lomurno@mail.polimi.it
% \vspace{0.25cm}

% Andrea Romanoni, Politecnico di Milano \\
% andrea.romanoni@polimi.it
% \vspace{0.25cm}

% Matteo Matteucci, Politecnico di Milano \\
% matteo.matteuci@polimi.it
% \vspace{0.25cm}
% \end{center}

\begin{abstract}
This is a detailed description of the changes applied to the text in the resubmission of the paper in order to improve it with respect to the weaknesses highlighted by the anonymous reviewers. We take this opportunity to thank reviewers suggestions which have helped us in reshaping significantly the contribution which now is more clear and complete.
\end{abstract}

%\IEEEpeerreviewmaketitle

\section{Reviewer 4}
\textbf{Strength:} It is well written, and well reasoned, and the authors show a comprehensive background research and domain knowledge.

\textbf{Weaknesses:} There doesn't seem to be any novel contribution in the paper. Despite offering a well rounded study on how to combine two methods,  the main accomplishment is that it can improve results on one benchmark, and perhaps
marginally.

\begin{quote}\emph{%
As implicitly suggested by the reviewer, we have extended the evaluation of the comparison to Tanks and Temples benchmark in order to provide a more complete view on the experiments and provide better hints on the effectiveness of the Super-Resolution in improving MVS reconstructions.
}\end{quote}
There is also an assumption in the hypothesis
of the paper that might not hold true: the paper assumes
that the use of SISR can add details in the higher
resolution that can be useful for MVS, this is not
necessarily true.

\begin{quote}\emph{
With the new experiments from Tanks and Temples benchmark we show how reconstructions quality is related to images resolution.
In fact, reconstructing 3D models from downsampled versions of the original dataset leads to less accurate models than using higher resolutions.
}\end{quote}
SISR networks are highly dependant on the
dataset used for training, so unless the network was
trained on images of the same type, and more importantly
with the same resolution that the paper is targeting, the
SISR network most likely will not add much, and probably
that is why the bicubic scaling had comparable results.

\begin{quote}\emph{%
The paper was updated to address an ambiguity emerged from the reviewers comments: both the model based on Deep Learning and the bicubic upsampling are considered SISR techniques, but we deepen the use of the first as it represents the state-of-the-art in the SISR field.
The new experiments suggested by reviewers show that, given two versions of the same dataset, one in low-resolution LR of size WxH and one in high-resolution HR of size 2Wx2H, HR reconstruction always achieves much better scores than the LR version.
This answers the doubt about the assumption that adding input details improves 3D models, indeed, for both types of SISR with 2x scale factor, we have obtained better results compared with LR ones and at the same time very close to HR scores.
We agree that the training of the SISR-DL model has a great impact on the quality of the result and we assume that there is a wide improvement margin by performing fine-tuning or a complete training but still our results show how it is useful also with a general purpose training.
}\end{quote}

\paragraph{Justification} The paper is well written and thought, and has the potential of helping other papers achieve better results. But the idea is not groundbreaking nor the results very interesting. It should at least include results in more than one benchmark also.

\begin{quote}\emph{%
We are aware we are not proposing a new model, but as pointed out, the goal of this work is to propose an additional step by which create new MVS pipeline or improve existing ones down.
By extending the experimental part to the Tanks and Temples benchmark, we are expanding the pool of results with remarkable performances by applying SISR to images with low resolution paving the way for further studies on ad-hoc SISR methods capable to enhance MVS.
}\end{quote}

\section{Reviewer 2}
\textbf{Strengths:} I think that it is an interesting idea to evaluate how efficient and useful it is to apply a super-resolution technique to the input images before using a MVS algorithm. The paper is in general well written and easy to follow.

\textbf{Weaknesses:} My strongest critic is that there are no novel technical contributions in the paper. The proposed methods are straightforward combinations of off-the shelf super resolution and MVS methods. The motivation to study the
impact of super-resolution applied on input images for 3D
reconstruction is good, but technical contribution is low.

\begin{quote}\emph{%
We are aware that we are not proposing a classic technical contribution and accept the reviewer's criticism from this point of view. The intent of the paper is to create a link between two areas of research so far separated. Therefore, the proposed SR-MVS models are only a first example for a new tool and a starting point for improving the state-of-the-art in the MVS field.
Our aim is to prove with our findings this is a line of research it is worth pursuing.
}\end{quote}
The conclusion from the experimental evaluation is not
clear. In the end it seems that using or not
super-resolution and which super resolution method to use
depends a lot on the dataset. Maybe designing a new
super-resolution method that automatically adapts to the
input data for better 3D reconstruction could be an
interesting research direction. Also, because the results
depend on the method for super-resolution, experiments with
using other super-resolution methods would bee better.

\begin{quote}\emph{%
We agree with the reviewer's observation; we proceeded to modify the conclusion and enrich it with new experimental proofs.
We also agree with the comments relating to the next steps, which will surely be deepened in future works but which go beyond the purpose of this paper in which we limit ourselves to showing a type of classic super-resolution (bicubic interpolation) and one based on deep learning (DBPN) and to what extent they are beneficial to MVS.
}\end{quote}
In the experiments, the authors say that many datasets
could not be used because the input images are too high
resolution. What prevents the authors to downsample the
input images and use the downsampled images to test their
proposed method? Then it would be interesting to compare
the results obtained with the super resolution images with
those obtained with the ground truth high resolution
images. The point is to see how much artifacts are created
by the super-resolution algorithms.

\begin{quote}\emph{%
Thanks to the suggestions received, we applied the SR-MVS approach also to downsampled version of Tanks and Temples, obtaining a set of LR and HR images of the benchmark. By applying bicubic-based and deep-learning-based super-resolution to the LR images, we obtained reconstructions with scores much better than the 3D LR models and very close to the original HR ones.
As for the artifacts of the SR, these are easy to find in the starting images and become less sharp continuing in the pipeline.
It is possible to identify them, for instance, as distortions or holes in the textureless regions of 3D reconstructions from MVS PatchMatch algorithms.
}\end{quote}
I guess that there is a trade-off between processing time
and using super-resolution images as input. This should be
discussed, and the improvements in accuracy when using
super-resolution images should be balanced by the increase
in computational time.

\begin{quote}\emph{%
We agree that a temporal analysis can provide very interesting information, and we confirm that there is a kind of proportionality between the size of the input and the reconstruction time. We decided to exclude this information from the paper experiments given the heterogeneity of the input which varies by starting size, number of images and channels and by the different nature of the MVS algorithms proposed.
We believe that a comparison of this type requires a very thorough work and that it would have diverted attention from the main problem that this document aims to solve.
However, on an Intel(R) Xeon(R) CPU E5-2630 v4 @ 2.20GHz with an Nvidia GTX 1080Ti, the bicubic interpolation requires a fraction of second for image while the Deep Back-Projection Network on average requires between 2 and 10 seconds; the 3D reconstruction process is heavily affected by the number of input images; from the experiments carried out over Tanks and Temples on average SR reconstructions have required 2-3 times the time required for low-resolution ones.
}\end{quote}

\paragraph{Rating}: The motivation of the paper is interesting, but the technical contribution is low and the experimental evaluation does not allow to answer the question of the paper: “is it better to use super-resolution algorithm before applying MVS method?”. Also, some additional experiments could have been done.

\begin{quote}\emph{%
We have enriched the experimental pool with Tanks and Temples benchmark evaluation to answer the reviewer doubts.
We also reformulated the explanation of the results by focusing on the technical contribution provided and on the key points of our approach in the MVS field.
}\end{quote}

\section{Reviewer 3}
\textbf{Rating:} The authors proposed a completeness of model reconstruction by using super-resolution. The evaluation results demonstrate that the proposed method works well for
textured scenes. I suggest giving more details of
explanation of the proposed method.

\begin{quote}\emph{%
We agree with the reviewer's critic and for this reason we have enriched the experimental pool with another benchmark and discussed these new results.
We would like to clarify that the methods used are aimed at studying the effectiveness of SISR in MVS pipelines and that they do not represent the core of the paper.
}\end{quote}
It is not clear how to
design the deep back projection network to generate SISR.

\begin{quote}\emph{%
We did not elaborate on the explanation about the deep back-projection network (DBPN) design since this model has not been realized by us.
It is the SISR model built and provided by Haris \etal which is publicly available on GitHub (https://github.com/alterzero/DBPN-Pytorch).
}\end{quote}
In the evaluation results, why some low-resolution images
provide better performance? The outdoor environment
situations are different, for example, city road, highway,
urban. It is an insufficient evaluation result to apply the
proposed method to the outdoor scene applications.

\begin{quote}\emph{%
According with reviewer suggestions, we extended the proposed approach to other indoor and outdoor sequences demonstrating the connection between input images and 3D model qualities. The reason why textureless low-resolution sequences lead to better 3D models is related with the nature of both the SISR and the MVS algorithms used: PatchMatch algorithms suffer for the presence areas poor in details, SISR may produce artifacts. We shown also how CasMVSNet, the DL-MVS algorithm used in our experiments, is instead able to exploit SISR in both indoor/outdoor and textured/textureless scenarios.
}\end{quote}


% \bibliographystyle{IEEEtranS}
% \bibliography{biblio.bib}

%\end{document}
